PANDORA: A Parallel Dendrogram Construction Algorithm for Single Linkage Clustering on GPU

This paper presents \pandora, a novel parallel algorithm for efficiently constructing dendrograms for single-linkage hierarchical clustering, including \hdbscan. Traditional dendrogram construction methods from a minimum spanning tree (MST), such as agglomerative or divisive techniques, often fail to efficiently parallelize, especially with skewed dendrograms common in real-world data. \pandora addresses these challenges through a unique recursive tree contraction method, which simplifies the tree for initial dendrogram construction and then progressively reconstructs the complete dendrogram. This process makes \pandora asymptotically work-optimal, independent of dendrogram skewness. All steps in \pandora are fully parallel and suitable for massively threaded accelerators such as GPUs. Our implementation is written in Kokkos, providing support for both CPUs and multi-vendor GPUs (e.g., Nvidia, AMD). The multithreaded version of \pandora is 2.2$\times$ faster than the current best-multithreaded implementation, while the GPU \pandora implementation achieved 6-20$\times$ on \amdgpu and 10-37$\times$ on \nvidiagpu speed-up over multithreaded \pandora. These advancements lead to up to a 6-fold speedup for \hdbscan on GPUs over the current best, which only offload MST construction to GPUs and perform multithreaded dendrogram construction.

==> 05_analysis.tex <==
\subsection{ Optimality of $\alpha$-contraction}\label{sec:analysis}
% \subsection{Proof of correctness}
In this section, we will demonstrate the correctness of the algorithm and the
optimality of the edge contraction using $E_{\alpha}$ for \cref{algm:alphatree}.
The proof proceeds as follows:
\begin{itemize}
  

  \item  First, we define the \textit{Lowest Common Dendrogram Ancestor (LCDA)}
  as the earliest shared ancestor edge in the dendrogram for any two given edges
  (Section \ref{sec:DendroEdgeContraction} and Definition \ref{def:lcda}).
  %  The
  % proof introduces the concept of the \textit{Lowest Common Dendrogram Ancestor
  % (LCDA)}, which represents the first common ancestor edge in the dendrogram two
  % given edges \Cref{sec:DendroEdgeContraction} and Definition \ref{def:lcda}).
  
  \item We then present a theorem connecting the LCDA to the minimum spanning
  tree's structure, stating that the LCDA of two edges corresponds to the edge
  with the smallest rank along the path connecting them in the tree (Theorem
  \ref{thm:lcda2path}).

  
  % The proof establishes a theorem that connects the LCDA to the structure of the
  % minimum spanning tree. Specifically, the theorem states that the LCDA of two
  % edges is the edge with the smallest rank along the path connecting the two
  % edges in the tree (Theorem \ref{thm:lcda2path}).
  
  \item Next, we examine the effects of edge contraction on dendrogram structure
  and introduce \textit{cluster hierarchy preserving edge contraction}, an edge
  contraction that maintains the original tree's dendrogram ancestry properties
  (Definition \ref{def:dendroContraction}). We provide necessary and sufficient
  conditions for an edge contraction to preserve cluster hierarchy.

  
  \item We prove the correctness of our algorithm (Algorithm
  \ref{algm:alphatree}) for generating dendrograms through edge contraction,
  demonstrating that contracting $\alpha$-edges satisfies the conditions
  required for the algorithm's correctness (Theorem \ref{thm:correctness}).
  \item Finally, we establish the optimality of $\alpha$-Contraction, the contraction
  of $\alpha$-edges, by presenting lemmas that indicate its necessity and
  sufficiency for the algorithm's correctness (Theorem \ref{thm:optimal} and
  Lemmas \ref{lem:necessary} and \ref{lem:sufficient}). 
  % The proof establishes
  % the correctness of the algorithm (Algorithm~\ref{algm:alphatree}) for
  % generating dendrograms using edge contraction. The algorithm is proven to be
  % correct if the edge contraction used is cluster hierarchy preserving. The
  % proof shows that contracting $\alpha$-edges satisfies the necessary and
  % sufficient conditions for the correctness of the algorithm (Theorem
  % \ref{thm:correctness}).
  % \item The proof concludes by demonstrating the optimality of $\alpha$-Contraction,
  % which is the contraction of $\alpha$-edges. The proof provides lemmas that
  % show that $\alpha$-Contraction is both necessary and sufficient for the
  % correctness of the algorithm (Theorem \ref{thm:optimal} and Lemmas
  % \ref{lem:necessary} and \ref{lem:sufficient}).
\end{itemize}

We connect the concepts of LCDA, edge contraction, and
dendrogram structure to establish the correctness and optimality of the
algorithm for generating dendrograms. 

% The proof introduces the Lowest Common Dendrogram Ancestor (LCDA), the nearest
% common ancestor edge in a dendrogram for two given edges. The LCDA concept is
% essential for comprehending the dendrogram's structure and edge relationships.

% We then establish a theorem linking the LCDA to the structure of the minimum
% spanning tree. This theorem asserts that the LCDA of two edges corresponds to
% the smallest-ranked edge along the path connecting these edges in the tree.

% Next, we explore the impact of edge contraction on dendrogram structure,
% presenting the notion of "cluster hierarchy preserving edge contraction." This
% type of edge contraction maintains the ancestry properties in the original
% tree's dendrogram. We provide conditions for an edge contraction to preserve the
% cluster hierarchy.

% Subsequently, we prove the correctness of the algorithm
% (Algorithm~\ref{algm:alphatree}) for generating dendrograms through edge
% contraction. If the edge contraction is cluster hierarchy preserving, the
% algorithm is correct. We demonstrate that contracting $\alpha$-edges fulfills
% the conditions for algorithm correctness.

% Finally, we showcase the optimality of $\alpha$-Contraction, which involves
% contracting $\alpha$-edges. We offer lemmas proving that $\alpha$-Contraction is
% both necessary and sufficient for the algorithm's correctness, indicating that
% it is the optimal method for generating accurate dendrograms using edge
% contraction.

% In summary, this proof connects the LCDA, edge contraction, and dendrogram
% structure concepts to establish the algorithm's correctness and optimality for
% generating dendrograms.


% To accomplish this, we first
% define several useful abstractions that help to express the underlying structure
% and interrelation of the edge-contraction with the dendrogram structure. We
% state and prove key results that capture the interrelation theorems that will
% enable us to prove the correctness and optimality of the $\alpha$-tree.
\iffalse
\subsection{Connecting the Dendrogram and the Tree structure}
We begin by defining the Lowest Common Dendrogram Ancestor (LCDA) of two edges
within a tree, a vital concept in our proof.

\begin{definition}[\lcdaexpanded]
\label{def:lcda}
    % \textbf{\lcdaexpanded:}
    Let $e_i$ and $e_j$ be two edges in a tree $T$.  We define the Lowest Common
    Dendrogram Ancestor of $e_i$ and $e_j$, denoted as $\lcda{e_i}{e_j}$ as
    follows. 
    \[
    \lcda{e_i}{e_j} \defined  \underset{e \in \ancshort{e_{i}} \cap \ancshort{e_{j}} }{\arg\max} \rank{e}
    \] 
    %
    If $e_{i} \in \ancestors{e_j}$, then $\lcda{e_i}{e_j} = e_i$ and vice versa. In other words,
    \begin{equation}
    \label{eq:lcda2anc}
    e_{i} \in \ancestors{e_j} \iff \lcda{e_i}{e_j} = e_i
    \end{equation}
\end{definition}

% \todo{add a figure of the definition of LCDA}

% explain in simple words what the LCDA is


%give a preface for the following theorem
Next, we present a theorem that establishes a relationship between the Lowest
Common Dendrogram Ancestor and the structure of the minimum spanning tree. 

\begin{theorem}
    \label{thm:lcda2path}
    Let $e_i$ and $e_j$ be any two edges in a tree $T$, then $\lcda{e_i}{e_j}$,
    will be the edge with the least rank in $\spath{e_i}{e_j}$.
    \begin{equation}     
    \label{eq:lcda2path}
    \lcda{e_i}{e_j} = \underset{e \in \spath{e_i}{e_j}}{\arg\min} \rank{e}.
    \end{equation}
\end{theorem}

Unlike \cref{def:lcda}, this \cref{eq:lcda2path} does not require information
about dendrogram ancestors of either edge. 
% explain in simple words what the LCDA is
% \todo{Add proof of the theorem}

The \cref{thm:lcda2path} allows us to understand structure of dendrogram in
terms of paths and adjacency structure of the tree. We give two corollaries of
the theorem to helps to demystify the relationship between the LCDA and the
dendrogram structure.

\begin{corollary}
    \label{cor:anc2path}
    If  $e_i$ has the smalllest rank in $\spath{e_i}{e_j}$, if and only if $e_{i}$ is a
    dendrogram ancestor of $e_j$.
    \begin{equation}
        \rank{e_i} {=} \underset{e \in \spath{e_i}{e_j} }{\min\rank{e}} \iff  e_{i} \in \ancestors{e_j}
    \end{equation}
\end{corollary}


\begin{corollary}
    \label{cor:anc2inc}
    If two edges $e_i$ and $e_j$ if they share a common vertex in $T$, and
    $i{<}j$ then $e_{i} \in \ancestors{e_j}$. 
    \begin{equation}
    \label{eq:anc2inc}
        \left\{ e_i, e_j \right\} \in \textsf{Incident}(v) \ i<j \implies e_{i} \in \ancestors{e_j}
    \end{equation}
\end{corollary}

\subsection{ Properties of the Edge Contraction's Dendrogram}
\label{sec:DendroEdgeContraction}
In this section, we seek to establish how edge contraction affects the
dendrogram. Specifically, we will show that under certain edge contractions
preserve the ancestory properties in the dendrogram of the original tree. We
characterize these contractions by providing neccessary and sufficient
conditions for the edge contractions.


\begin{theorem}[Dendrogram Ancestor Preservation in Edge Contraction]
\label{thm:lcda2lcda}
Let $T$ and $T_c=(V_c, E_c)$ be a tree and it's an edge contraction, respectively, and $e$ and
$f$ be any two edges present in both.  
Then $\lcda[T]{e}{f} = \lcda[T_c]{e}{f}$ if and only if $\lcda[T]{e}{f} \in E_c$.
\begin{equation}
\label{eq:lcda2lcda}
\lcda[T]{e}{f} = \lcda[T_c]{e}{f} \iff \lcda[T]{e}{f} \in E_c
\end{equation}

\textbf{Proof:}
Let us denote $g = \lcda[T]{e}{f}$. We will prove the theorem by considering two cases:
\begin{enumerate}
    \item (Only if) By definition, $\lcda[T_c]{e}{f}$ is an edge in $E_c$. If $g
    \notin E_c$, then $g \neq \lcda[T_c]{e}{f}$.

    \item  (If) Recall that $g$ is the edge with the minimum rank in the path between
    edges $e$ and $f$ in tree $T$, denoted as $\spath[T]{e}{f}$. The path
    contracted path, denoted as $\spath[T_c]{e}{f}$, is a
    subsequence of $\spath[T]{e}{f}$, e.g.:
    \[
        \spath[T_c]{e_i}{e_j} \subseteq \spath[T]{e_i}{e_j}.
    \]
    Moreover, if edge $g$ is present in $E_{c}$, it will also be present in
    $\spath[T_c]{e}{f}$. As $g$ has the minimum rank among the edges in
    $\spath[T]{e}{f}$, it will have the least rank in any subsequence of
    $\spath[T]{e}{f}$, including $\spath[T_c]{e_i}{e_j}$.
    Therefore, we can conclude that:
    \[
        g = \underset{e \in \spath[T_c]{e_i}{e_j}}{\arg\min} \rank{e} = \lcda[T_{c}]{e}{f}.
    \]
\end{enumerate}
\end{theorem}

\begin{corollary}[Dendrogram Ancestor Preservation in Edge Contraction]
\label{cor:anc2anc}
    Given a tree
    $T$, and its edge contraction $T_c$, let $e$ and $f$ be two edges present in
    both $T$ and $T_c$. If $e$ is a dendrogram ancestor of $f$ in $T$, then $e$
    will be a dendrogram ancestor of $f$. However, the converse is not always true.
    
    \begin{proof}
    If $e$ is a dendrogram ancestor of $f$, then $\lcda[T]{e}{f} = e$. Since
    $e$, $f$ and $\lcda[T]{e}{f}=e$ are present in $E_{c}$, Hence, by
    \cref{thm:lcda2lcda}, we can conclude that $\lcda[T_c]{e}{f} = e=
    \lcda[T]{e}{f}$. Moreover, from \cref{eq:lcda2anc}, $\lcda[T_c]{e}{f} = e$
    also implies that $e$ is a dendrogram ancestor of $f$ in $T_c$. Hence, 
    \begin{equation}
        \label{eq:ancContraction}
        e \in \ancestors[T]{f} \implies e \in \ancestors[T_c]{f}
    \end{equation}
\end{proof}
\end{corollary}


The converse of \cref{cor:anc2anc} is not always true. Consider a chain
of three edges, $[e_i, e_k, e_j]$, such that $k < i < j$. The edge $e_k$ has the
least rank and is the LCDA of $e_i$ and $e_j$: $\lcda{e_i}{e_j} = e_k$. In this
case, $e_i$ and $e_j$ are not dendrogram ancestors of each other. However, if we
contract edge $e_k$, in the contracted tree, $e_i$ will become a dendrogram
ancestor of $e_j$ in the dendrogram for the contracted tree, showing that the
converse is not always true.

\newcommand{\preservCAP}{ Cluster Hierarchy Preserving}
\newcommand{\preservSM}{ Cluster-hierarchy preserving}
\textbf{Implications of \cref{cor:anc2anc}}: 
As implied by \cref{cor:anc2anc}, it is not always possible to infer accurate
dendrogram information from the dendorgram of any arbitrary edge contraction
$E_c$. Consequently, \cref{algm:alphatree} may not produce correct results for
all edge contractions. This observation motivates the importance of identifying
\preservCAP~ edge contractions.

%
% In this context, 
\subsection{\preservCAP~Edge Contraction}
% could be cluster hierarchy preserving edge contraction
%
In the following section, we define and characterize which edge contractions can
be used with \cref{algm:alphatree}. Furthermore, we establish that $\alpha$-edges
represent the optimal choice for edge contractions in \cref{algm:alphatree}.
\begin{definition}[\preservSM~Edge Contraction]
\label{def:dendroContraction}
% \textbf{\preservSM~Edge Contraction:}\\
We call an edge contraction $T_c$, \preservSM~if for any $e, f
\in E_c$, $e$ is a dendrogram ancestor of $f$ in $T_c$ if and only if $e$ is
a dendrogram ancestor of $f$ in $T$. 
\begin{equation}
    \label{eq:dendroPreContraction}
    e \in \ancestors[T_{c}]{f} \implies e \in \ancestors[T]{f} 
\end{equation}
\end{definition}
%
%

\begin{theorem}
An edge contraction $E_c$ is \preservSM~if for all edges $e$ and
$f \in E_c$, $\lcda[T]{e}{f} \in E_c$.
    
\begin{proof}
We aim to demonstrate that if $e$ is an ancestor of $f$ in the dendrogram of
$T_c$, then $e$ is also an ancestor of $f$ in the original dendrogram $T$. 
Since $e$ is an ancestor of $f$ in  $T_c$, we have:
\[
\lcda[T_{c}]{e}{f} = e
\]
%
\textbf{To prove:} Our goal is to show that $e$ is an ancestor of $f$ in the original dendrogram
$T$, which is equivalent to proving:
\[
\lcda[T]{e}{f} = e
\]
%
According to the statement of the theorem, we have $\lcda[T]{e}{f} \in E_c$.
From \cref{eq:lcda2lcda}, if $\left\{e, f, \lcda[T]{e}{f}\right\} \in E_c$,
then:
\[
\lcda[T]{e}{f} = \lcda[T_c]{e}{f} = e
\]
Consequently, $\lcda[T]{e}{f} = e$, proving that $e$ is an ancestor of $f$ in
the original dendrogram $T$.
\end{proof}
\end{theorem}

\subsection{Correctness of \cref{algm:alphatree}} 
\label{sec:correctness}
We establish the correctness of Algorithm~\ref{algm:alphatree}  in two steps.
First, we characterize the edge contractions that guarantee the correct results
for \Cref{algm:alphatree}. These conditions are formally stated in
Theorem~\ref{thm:correctness}. Second, we demonstrate that contracting
$\alpha$-edges---defined in \cref{def:alphaedge}, is optimal. Specifically, we
show that contracting $\alpha$-edges satisfies the necessary and sufficient
conditions for the correctness of Algorithm~\ref{algm:alphatree}. 
%
\begin{theorem}
\label{thm:correctness} 
\Cref{algm:alphatree} produces a correct
dendrogram for a given edge contraction $E_c$ if for any edges $e \in E$,
the edge contraction $E_c \cup e$ is a \preservSM~edge contraction.
\end{theorem}
%
We omit the full proof of \cref{thm:correctness} as it does not offer any
crucial insight beyond what has been discussed so far. However, we provide a
brief outline of the steps involved in the proof. To prove the theorem's
correctness, we must demonstrate that for all edges $e$, the parent of edge
$P(e)$ computed using \Cref{algm:alphatree} is equal to the correct parent
$P^{*}(e)$. To achieve this, we show that:
%
\begin{itemize}
    \item $e$ and $P^{*}(e) \notin E_{c}$ are mapped to the same branch of the
    contracted dendrogram.
    \item No other edge $f$ exists, such that $f$ is mapped to the same branch
    as $e$ and $\rank{P^{*}(e)} > \rank{f} > \rank{e}$.
\end{itemize}

\newcommand{\warning}[1]{\textcolor{red}{\textbf{#1}}}
\subsection{Optimality of $\alpha$-Contraction}
\label{sec:alphaoptimal}
Finally, we show that the optimality of $\alpha$-Contraction for
\cref{algm:alphatree}, i.e., tree contraction using $\alpha$-edges $E_{\alpha}$
as defined in \cref{def:alphaedge}, is necessary and sufficient for producing a
correct dendrogram.

\begin{theorem}
\label{thm:optimal}
    $\alpha$-Contraction $E_{\alpha}$  is neccessary and sufficient
    to satisfy correctness conditions specified by \cref{thm:correctness}.
\end{theorem}
%
% - we prove it in following steps: 
%
\begin{lemma}[Necessary Condition]
\label{lem:necessary}
\textit{(Necessary:)} For every $\alpha$-edge $e_{\alpha} \in E_{\alpha}$, there
exist edges $e_{r}$ and $e_{s}$ such that $\lcda[T]{e_{r}}{e_{s}} = e_{\alpha}$.
\begin{proof}
Let $e_{\alpha} = (v,u)$ be an arbitrary $\alpha$-edge in $E_{\alpha}$.
By definition, the maximum rank of edges incident to vertices $v$ and $u$ is
greater than $\rank{e_{\alpha}}$. Let $e_{vx}$ and $e_{ux}$ be the edges in
$\text{Incident}(v)$ and $\text{Incident}(u)$, respectively, with maximum rank.
By construction, we have $\rank{e_{vx}} > \rank{e_{\alpha}}$ and $\rank{e_{ux}}
> \rank{e_{\alpha}}$. We claim that $\lcda[T]{e_{ux}}{e_{vx}} = e_{\alpha}$.
This follows from $\lcda[T]{e_{ux}}{e_{vx}}$ is the edge with minimum rank in
$\spath[T]{e_{vx}}{e_{ux}} = \left [ e_{vx}, e_{\alpha},e_{ux}  \right ]$.
\end{proof}
\end{lemma}

\begin{lemma}[Sufficient Condition]
\label{lem:sufficient}
If $e_x \notin E_{\alpha}$, then $e_x$ cannot be the lowest common
dendrogram ancestor edge of any two edges $e_r$ and $e_s$.
%
\begin{proof}
    Let $e_x = (v,u)$ be an edge not in $E_{\alpha}$. By the definition of an
    $\alpha$-edge, $e_x$ has the largest rank in either $\text{Incident}(v)$ or
    $\text{Incident}(u)$. Without loss of generality, assume $e_x$ has the
    largest rank in $\text{Incident}(v)$.Consider a path in tree $T$ containing
    $e_x$, given by 
    %
    \[
        \spath[T]{e_r}{e_s} = \left [e_r, \dots, e_v,
    e_x, e_u, \dots, e_s \right ]
        \], 
        where $e_v \in \text{Incident}(v)$ and $e_u \in
    \text{Incident}(u)$. Since $e_x$ has the largest rank in
    $\text{Incident}(v)$ hence $\rank{e_v} < \rank{e_x}$. We conclude that
    $e_{x}$ can have the smallest rank in any $\spath[T]{e_r}{e_s}$, hence
    $\lcda[T]{e_r}{e_s} \neq e_x$ for any two edges $e_r$ and $e_s$.
\end{proof}
\end{lemma}
\fi 


==> Makefile <==
all: single-blinded

# IEEEtran.cls:
	# wget http://mirrors.ctan.org/macros/latex/contrib/IEEEtran/IEEEtran.cls

metadata.tex: metadata.json
	python3 meta2tex.py  metadata.json IEEE double-blind

single-blinded: metadata.tex
	pdflatex main.tex
	bibtex main
	pdflatex main.tex
	pdflatex main.tex

.PHONY: clean
clean:
	rm -f *.aux *.log *.blg *.bbl *.out *.ps *.toc *.dvi *.xcp

arxiv:
	pdflatex main.tex
	bibtex main
	COPYFILE_DISABLE=1 tar -k -cvf arxiv.tar \
		orcidlink.sty \
		main.bbl \
		*.tex \
		hdbscan.sty \
		experiments/*.pdf \
		figs/*.pdf \
		figs/*.png \
		plots/*.pdf


==> algs/aAlphaTree.tex <==
% alphaEdges = $E_{\alpha}$
% $ T_{\alpha} = $T_{\alpha}$
% \xbetatree = $ \mathcal{D}_{\beta}$
% alphaParents = $\mathcal{D}_{\alpha}$
\newcommand{\xbetatree}{\ensuremath{\mathcal{D}_{\beta}}}
\newcommand{\xalphatree}{\ensuremath{\mathcal{D}_{\alpha}}}
\newcommand{\xalphaedges}{\ensuremath{E_{\alpha}}}
\newcommand{\xalphamst}{\ensuremath{T_{\alpha}}}
\newcommand{\xmst}{\ensuremath{T}}
\newcommand{\xmaxincident}{\ensuremath{\max \textsf{Incident}}}
\begin{algorithm}
\caption{Find $\alpha$-tree recursively}\label{alg:ralphatree}
\begin{algorithmic}[1]
\Procedure{rAlphaTree}{$T$, $level$}
\State $\eta \overset{\underset{\mathrm{def}}{}}{=}$ Max recursion level  
\State $\xalphaedges \gets$ \Call{Compute\ $\alpha${-}Edges}{$T$}

\State $T_{\alpha} \gets$ \Call{Compute\ Euler\ Tour}{$\xalphaedges$, $T$}
\If{$level < \eta$}
    \State $\xbetatree \gets$ \Call{rAlphaTree}{$\xalphaedges$, $level + 1$}    
    \State $\xalphatree \gets$ \Call{Compute\ Dgram($\alpha$)}{$\xalphaedges$, $\xbetatree$}
\Else
    \State $\xalphatree \gets$ \Call{Compute\ Dgram(Base)}{$\xalphaedges$}
\EndIf
\State \textbf{return} $\xalphatree$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> algs/alphaDgram.tex <==
\newcommand{\xbranchedge}{\ensuremath{\mathcal{B}}}
\begin{algorithm}
\caption{Compute Dendrogram using \alphatree}\label{alg:cap}
\begin{algorithmic}[1]
\Procedure{computeDendrogramUsing\xalphatree}{$T, \xalphatree$}
\State $n_e \gets |T|$ 
\State $\xbranchedge \gets$ \text{list of length $n_e$ of pairs integers}
\For{$k \in 0 {:} n_e {-} 1$} \textbf{ in parallel}
\State $P_{\alpha} \gets$ \Call{\findalphaparent}{$e_{k}$,$\xmst$, $\xalphatree$ }
% \State $\text{branch} \gets 2P_{\alpha}$
% \If  $e_{k} \in \innerside(P_{\alpha})$
%     \State $\text{branch} \gets \text{branch} + 1$
% \EndIf
\State $\text{branch} \gets $  \Call{{$\alpha$}{-}\textsf{ParentToBranch}}{$P_{\alpha}$}
% \State $\xbranchedge[e_{k}] \gets$ \Call{\xbranchedge_t}{$\xalphatree.computeBranch(e_{k},T), e_{k}$}
\State $\xbranchedge[k] \gets \binom{\text{branch}}{k}$
\EndFor
\Statex \Comment{Sort $\xbranchedge$ by branch, then by index}
\State \Call{sort}{$\xbranchedge$} 
% \State $parent \gets$ \Call{vector<int>}{$n_e, {-}1$}
\For{$b_{e} \gets 1 {:} n_e {-} 1$} \textbf{in parallel}
\State $\text{my branch} \gets \xbranchedge[b_{e}].branch$
\State $k \gets \xbranchedge[b_{e}].index$
\If{$\xbranchedge[b_{e} {-} 1].branch == \text{my branch}$}
\State $\mathcal{D}(e_{k}) \gets \xbranchedge[b_{e} {-} 1].e_{k}x$
\Else
\State $\mathcal{D}(e_{k}) \gets$ \Call{\textsf{BranchTo}{$\alpha$}-\textsf{Parent}}{ my branch}
\EndIf
\EndFor
\State \textbf{return} $\mathcal{D}$
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> algs/alphaParent.tex <==
\newcommand{\xmybridge}{\ensuremath{ v_{\alpha}}}
\newcommand{\alphaparentsearch}{$\alpha{-}$\textsf{ParentSearch}\xspace}
\newcommand{\findalphaparent}{$\textsf{Find}\alpha{-}$\textsf{Parent}\xspace}
% \begin{algorithm}
% \caption{Find $\alpha$-parent}\label{alg:cap}
% \begin{algorithmic}[1]
% \Procedure{Find-Alpha-Parent}{$e_{k}, \xalphaedges, \alphaAncestors$}
% \If{$k < \xalphaedges[0]$}
% \State \Return{-1} \Comment{The top branch}
% \EndIf
% \State $\xmybridge \gets \xalphamst.Insert(\xmst .entry(e_{k}), \xmst .exit(e_{k}))$
% \If{$\xalphaedges[\xalphamst.maxIdxBridge(\xmybridge)] < e_{k}$}
% \State \Return{$\xalphamst.maxIdxBridge(\xmybridge)$}
% \EndIf
% \State \Return{$\alphaTreeBottomUpParentSearch(e_{k}, \xalphamst.maxIdxBridge(\xmybridge), \xalphaedges, \xalphatree)$}
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}
    \caption{Find $\alpha$-parent}\label{alg:cap}
    \begin{algorithmic}[1]
    \Procedure{\findalphaparent}{$e_{k}$, $\xmst $}
    \If{$e_{k} < \xalphaedges[0]$}
        \State \textbf{return} -1 \Comment{The top branch}
    \EndIf
    % \If{$ e_{k} \in \xalphaedges$}
    %     \State \textbf{return} $\alphaParents[invAlphaEdges[e_{k}]]$
    % \EndIf
    \State $\xmybridge \gets$ \Call{Insert}{$\xalphamst$, $e_{k}$}
    % \If{$\xalphaedges[\xalphamst.maxIdxBridge(\xmybridge)] < e_{k}$}
    \State $\Delta_{k} \gets \xmaxincident_{\alpha}(\xmybridge)$
    \If {$\Delta_{k} < k$}
        \State \textbf{return} $\Delta_{k}$
    \EndIf
    \State \textbf{return} \Call{\alphaparentsearch}{$e_{k}$, $\Delta_{k}$, $\xalphatree$}
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    
    \begin{algorithm}
    \caption{Find $\alpha$-parent (Bottom-up)}\label{alg:cap}
    \begin{algorithmic}[1]
    \Procedure{\alphaparentsearch}{$e_{k}$, $\Delta$, $\xalphatree$}
    \State $l_{max} \gets \log \text{height}(\xalphatree) $
    \State $\Delta_{new} \gets \xalphatree(\Delta)$
    \For{$l \gets 1$\ \textbf{to}\ $l_{max}$}
        \If{$\xalphatree^{2^l} (\Delta) < 0$ \textbf{or} $\xalphatree^{2^l} (\Delta) < e_{k}$}
            \State \textbf{return} \Call{\alphaparentsearch}{$e_{k}$, $\Delta_{new} $, $\xalphatree$}
            \State $\Delta_{new} \gets \xalphatree^{2^{l}} (\Delta)$
        \EndIf
    \EndFor
    \State \textbf{return} \Call{\alphaparentsearch}{$e_{k}$, $\Delta_{new}$, $\xalphatree$}
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}

==> algs/dendrogramUsingContraction_alt.tex <==
\begin{algorithm}[H]
  \caption{\label{algm:alphatree}Dendrogram construction using contractions for a given MST $T = (V, E)$}
\begin{algorithmic}[1]
\State $E_F \gets \textsf{FindFEdges}(T)$
\State $T_C \gets \textsf{ComputeEdgeContraction}(T, E_F)$
\State $D_C \gets \textsf{ComputeDendrogram}(T_C)$
\For{$e$ in $E_F$}
    \State $P_C(e) \gets \textsf{ComputeCParent}(e, D_C)$
    \State $\textsf{Chain}(e) \gets \textsf{Map to}\ \alpha\textsf{CChain}(e)$
\EndFor
\State $C_{\alpha} \leftarrow \{[\textsf{Chain}(e), e], \forall e \in E\}$
\State $\text{Sort } C_{\alpha} \text{ by first and second element}$
\For{$e$ in $E$}
    \State $\text{Compute } P(e) \text{ using sorted } C_{\alpha}$
\EndFor
\Return $P$
\end{algorithmic}
\end{algorithm}


==> algs/dfs.tex <==


        
        \newcommand{\incMatMST}{\text{IncMatMST}}
        \newcommand{\EdgeList}{\text{EdgeList}}
        \newcommand{\DFS}{\text{DFS}}
        \newcommand{\mstEulerEntry}{\text{Entry}}
        \newcommand{\mstEulerExit}{\text{Exit}}
        
        \begin{algorithmic}
        \Function{eulerTour}{$\incMatMST$, $\EdgeList$}
            \State $time \gets 0$
            \State $root \gets 0$
            \State $\mstEulerEntry \gets \text{zeros}((|E|), dtype=int)$
            \State $\mstEulerExit \gets \text{zeros}((|E|), dtype=int)$
            % \State $\mstEulerEntryExit \gets (\mstEulerEntry, \mstEulerExit)$
            \State let $(v,u) \gets $
            \State $time \gets \DFS(\EdgeList[root].first.first, time, root, \mstEulerEntryExit)$
            \State $\mstEulerEntry[root] \gets time$
            \State $time \gets time + 1$
            \State $time \gets \DFS(\EdgeList[root].first.second, time, root, \mstEulerEntryExit)$
            \State $\mstEulerExit[root] \gets time$
            \State $time \gets time + 1$
            \State \Return $\mstEulerEntryExit$
        \EndFunction
        
        \Function{DFS}{$vtxId$, $time$, $bridgeEdge$, $\mstEulerEntryExit$}
            \State $k \gets 0$
            \While{$k < \incMatMST.numIncidentEdge(vtxId)$}
                \State $kthEdge \gets \incMatMST.k_thIncidentEdge(vtxId, k)$
                \If{$kthEdge == bridgeEdge$}
                    \State $k \gets k + 1$
                    \State \textbf{continue}
                \EndIf
                \State $\mstEulerEntry[kthEdge] \gets time$
                \State $time \gets time + 1$
                \State $utx \gets \EdgeList[kthEdge].first.first + (\EdgeList[kthEdge].first.second - vtxId)$
                \State $time \gets \DFS(utx, time, kthEdge, \mstEulerEntryExit)$
                \State $\mstEulerExit[kthEdge] \gets time$
                \State $time \gets time + 1$
                \State $k \gets k + 1$
            \EndWhile
            \State \Return $time$
        \EndFunction
        \end{algorithmic}
        

==> algs/edgeList2incidence.tex <==
\begin{algorithm}
\caption{Convert tree from edge list to Euler tour}\label{alg:cap}
\begin{algorithmic}[1]
\Procedure{ToEulerTour}{$E$}
    \State $n_e \gets |E|$
    \State $count \gets \{0\}_{n_e {+} 1}$
    \ForAll{$e \in E$} \textbf{in parallel}
        \State $[v, u] \gets e$
        \State $count[v] \gets count[v]{+}{+}$ \Comment{Atomic increment}
        \State $count[u] \gets count[u]{+}{+}$
    \EndFor
    \State $V_{ptr} \gets exclusivePrefixSum(count)$
    \State $I_{List} \gets \{\}_{2n_e}$
    \State $count \gets \{0\}_{n_e {+} 1}$
    \ForAll{$e \in E$} \textbf{in parallel}
        \State $[v, u] \gets e$
        \State $I_{List}[V_{ptr}[count[v]{+}{+}]] \gets e$
        \State $I_{List}[V_{ptr}[count[u]{+}{+}]] \gets e$
    \EndFor
    \State \Return $V_{ptr},\ I_{List}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> algs/weijaja.tex <==
\begin{algorithm}[H]  %%%% change the algorithm environment to algpseudocode 
\caption{Parallel List Ranking}\label{alg:parallel-list-ranking} 
\begin{algorithmic}[1]  %%%% comment the above line 
\State{Input: An array $\mathrm{S}$, containing successors of $n$ nodes and array $\mathrm{R}$ with ranks initialized to $1$} 
\State{Output: An array $\mathrm{R}$, containing the ranks of the nodes, such that $\mathrm{R[i]}$ is the rank of node $i$, for all $i$} 
\State{Local variables: An array $\mathrm{L}$, containing locations of the heads of sublists} 
\State{Initialization: $\mathrm{L[0]} = 0$, $\mathrm{L[s]} = n$} 
\For{$i = 1$ to $s-1$} 
\State{$\mathrm{L[i]} = \mathrm{random(0, n)}$} 
\EndFor %%%% add the endfor 
\For{$i = 1$ to $s-1$} 
\State{$\mathrm{L[i]} = \mathrm{L[i]} + \mathrm{L[i-1]}$} 
\EndFor %%%% add the endfor 
\State{$\mathrm{PrefixSum(L, s)}$} 
\State{$\mathrm{L[i]} = \mathrm{L[i]} + i$} 
\For{$i = 0$ to $n$} 
\State{$\mathrm{R[i]} = \mathrm{R[i]} + \mathrm{L[S[i]]}$} 
\EndFor %%%% add the endfor 
\State{$\mathrm{PrefixSum(R, n)}$} 
\State{Return $\mathrm{R}$} 
\end{algorithmic}
\end{algorithm}


% python code
% def list_rank(list,pointer,splitter):
% 	'''
% 	Step 1: Compute the location of the head of the list.
% 	Step 2: Select s random locations of X to split the list
% 	into s random sublists, where each random location
% 	provides a pointer to the head of a sublist. As we will
% 	see, the value of s will be selected to guarantee load
% 	balancing with high probability.
% 	Step 3: Using the standard sequential algorithm,
% 	compute the prefix sums of each sublist separately. All
% 	the sublists can be handled in parallel.
% 	Step 4: Compute the prefix sums of the list consisting
% 	exclusively of the splitters, where the successor of a
% 	splitter is the next splitter encountered when traversing
% 	the initial list.
% 	Step 5: Update the prefix value of each element of the
% 	array X by us
% 	'''
% 	# Step 1: Compute the location of the head of the list.
% 	head = list[0]
% 	# Step 2: Select s random locations of X to split the list
% 	# into s random sublists, where each random location
% 	# provides a pointer to the head of a sublist. As we will
% 	# see, the value of s will be selected to guarantee load
% 	# balancing with high probability.
% 	splitter = []
% 	for i in range(0,splitter):
% 		splitter.append(random.randint(0,len(list)-1))
% 	splitter = sorted(splitter)
% 	# Step 3: Using the standard sequential algorithm,
% 	# compute the prefix sums of each sublist separately. All
% 	# the sublists can be handled in parallel.
% 	sublist = []
% 	for i in range(0,splitter):
% 		sublist.append(list_rank(list[splitter[i]:splitter[i+1]],pointer,splitter))
% 	# Step 4: Compute the prefix sums of the list consisting
% 	# exclusively of the splitters, where the successor of a
% 	# splitter is the next splitter encountered when traversing
% 	# the initial list.
% 	splitter_rank = []
% 	for i in range(0,splitter):
% 		splitter_rank.append(list_rank(splitter[i],pointer,splitter))
% 	# Step 5: Update the prefix value of each element of the
% 	# array X by us
% 	for i in range(0,splitter):
% 		sublist[i] = sublist[i] + splitter_rank[i]
% 	return sublist

==> algs/wyllie.tex <==
% \begin{algorithm}
% \caption{Input: An array S, containing successors of n nodes and array R with ranks initialized to 1
% Output: Array R with ranks of each element of the list with respect to the head of the list}
% \begin{algorithmic}[1] 
%     \For{$i \in [1,n]$}
%     \While{$S[i]$ and $S[S[i]]$ are not the end of list}
%     \State $R[i] \leftarrow R[i] + R[S[i]]$
%     \State $S[i] \leftarrow S[S[i]]$
    
%     \EndWhile 
%     \EndFor
%     \end{algorithmic}
% \end{algorithm}


\begin{algorithm}
    \caption{Compute ranks of each node in a singly linked list}
    \label{alg1}
    \begin{algorithmic}[1] 
    \Function{ComputeRanks}{$S$}
    \State \textbf{Input:} An array $S$, containing successors of $n$ nodes and array $R$ with ranks initialized to 1
    \State \textbf{Output:} Array $R$ with ranks of each element of the list with respect to the head of the list
   
        \For{$i \in [1,n]$}
        \While{$S[i]$ and $S[S[i]]$ are not the end of list}
        \State $R[i] \leftarrow R[i] + R[S[i]]$
        \State $S[i] \leftarrow S[S[i]]$
        
        \EndWhile 
        \EndFor
        \EndFunction
        \end{algorithmic}
    \end{algorithm}
    
% \begin{algorithm}[h]
    
%     \caption{Parallel List Ranking}\label{alg:parallel-list-ranking}
%     \State{Input: An array S, containing successors of n nodes and array R with ranks initialized to 1}
%     \begin{algorithmic}[1]
%     \Procedure{ParallelListRanking}{$X, n$}
%     \State $head \leftarrow 0$
%     \State $s \leftarrow 10$
%     \State $Sublist\_head \leftarrow [0] * s$
%     \For{$i \leftarrow 0$ \textbf{to} $s$}
%         \State $Sublist\_head[i] \leftarrow random.randint(0, n)$
%     \EndFor
%     \State $Sublist\_prefix \leftarrow [0] * s$
%     \For{$i \leftarrow 0$ \textbf{to} $s$}
%         \State $Sublist\_prefix[i] \leftarrow prefixSum(X[Sublist\_head[i] : n], n/s)$
%     \EndFor
%     \State $splitters \leftarrow [0] * s$
%     \For{$i \leftarrow 0$ \textbf{to} $s$}
%         \State $splitters[i] \leftarrow X[Sublist\_head[i] - 1]$
%     \EndFor
%     \State $prefixSum(splitters, s)$
%     \For{$i \leftarrow 0$ \textbf{to} $n$}
%         \State $X[i].prefix \leftarrow X[i].prefix + splitters[-X[i].successor]$
%     \EndFor
%     \State \textbf{return} $X$
%     \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{Parallel List Ranking}\label{alg:parallel-list-ranking}
%     \begin{algorithmic}[1]
%     \State{Input: An array S, containing successors of n nodes and array R with ranks initialized to 1}
%     \State{Output: An array R, containing the ranks of the nodes, such that R[i] is the rank of node i, for all i}
%     \State{Local variables: An array L, containing locations of the heads of sublists}
%     \State{Initialization: L[0] = 0, L[s] = n}
%     \For{i = 1 to s-1}
%     \State{L[i] = random(0, n)}
%     \EndFor
%     \For{i = 1 to s-1}
%     \State{L[i] = L[i] + L[i-1]}
%     \EndFor
%     \State{PrefixSum(L, s)}
%     \State{L[i] = L[i] + i}
%     \For{i = 0 to n}
%     \State{R[i] = R[i] + L[S[i]]}
%     \EndFor
%     \State{PrefixSum(R, n)}
%     \State{Return R}
%     \end{algorithmic}
%     \end{algorithm}




==> tables/notation.tex <==
\begin{table}[th]
\centering
\ra{1.1}
% \rowcolors{2}{gray!25}{white}
% \begin{tabular}{@{}lll@{}}
        \begin{tabularx}{\columnwidth}{ll@{}}
                \toprule\midrule
                \textbf{Symbol} & \textbf{Description} \\
                \midrule
                $T$ & Minimum Spanning Tree (MST) with vertices $V$, edges $E$, and weights $W$ \\
                $n_{v}$ & Total vertices in the MST \\
                $n$ & Total edges in the MST, calculated as $n=n_{v} - 1$ \\
                $\Incident{v}$ & Edges incident to a vertex $v$ in $V$ \\
                $\maxIncident{v}$ & Edge with the highest weight incident to vertex $v$ \\
                $\edgeneighbor{e}$ & Edges adjacent to edge $e$, sharing a common vertex \\
                $P(v)$ & Parent of a vertex $v$ in the dendrogram, defined as $\maxIncident{v}$ \\
                $V \cup E$ & Vertices of the dendrogram, consisting of vertex and edge nodes from $T$ \\
                $\Edge{u}{v}$ & Directed edge in the dendrogram from node $u$ to node $v$ \\
                Leaf Edges & Edge nodes in the dendrogram with both children as vertex nodes \\
                Chain Edges & Edge nodes with one vertex node and one edge node as children \\
                $\alpha$-Edges & Edge nodes with no vertex nodes as children \\
                Chain & A sequence of non-$\alpha$ edges connected by parent-child relationships \\
                Skewness & Ratio of the dendrogram's height to its ideal height, $\log_{2} n$ \\
                $T_{c}$ & Contracted tree obtained by contracting a subset of edges $E_{c}$ \\
                $V_{c}$ & Vertices in the contracted tree, including new elements for merged supernodes \\
                $T_{\alpha}$ & $\alpha$-Tree, a tree formed by contracting non-$\alpha$ edges \\
                $\alpha$-vertex & Vertex in $T_{\alpha}$ representing multiple contracted vertices from $T$ \\
                \bottomrule
                \end{tabularx}
\caption{Notation for Minimum Spanning Tree}
\label{tab:MST-notation}
\end{table}
            


% \newcommand{\alphaedgeset}{\ensuremath{\mathcal{A}}\xspace}
% \newcommand{\alphaparent}[1]{\ensuremath{\mathcal{P}_{\alpha} \left\( #1 \right \)}\xspace}


% \begin{table}[]
% \centering
% \caption{List of symbols used}
% \label{tab:notation}
% \footnotesize
% \ra{1.1}
% \rowcolors{2}{gray!25}{white}
% \begin{tabular}{@{}lll@{}}
% \toprule\midrule
% Symbol type      & Symbol           & Description              \\
% \midrule
% %
% & $P$				& \#MPI processes \\
% & $P_{x}$,\ $P_{y}$,\ $P_{z}$	& Process grid dimensions						\\
% & $P_{xy}$			& $P_{x}\times P_{y}$ \# processes in $xy$ plane				\\
% & $p_{x}$,\ $p_{y}$,\ $p_{z}$	& Process coordinates						\\
% & $P_{r}(k)$			& $(k\mod P_{x})$-th process row					\\
% & $P_{c}(k)$			& $(k\mod P_{y})$-th process column					\\
% \multirow{-6}{*}{Process} 
% & $P_{kk}$			& Process that owns $A_{kk}$ block ($P_{kk} =P_{r}(k) \cap P_{c}(k) $)					\\
% % \todo{Define Desc{k}, Pkk, Prk, Pck}
% % \midrule
% % \multirow{4}{*}{\specialcell{Matrix \& \\ Indexing}}
% % &$A,\ L,\ U$& \specialcell{The input matrix $A$\\ and $LU$  factors}			\\
% % &$b$				& Right hand side							\\
%         % &		&									\\
%         % &		&									\\
% \midrule
% %
% & $E$		&  Elimination tree of $A$								\\
% & $S$		&  Top level separator of $E$								\\
% &$C_{1},\ C_{2}$&  Children etrees of $E$								\\
% &$Desc(k)$ 	& Descendants of node $k$ in $E$								\\
% \multirow{-5}{*}{Graphs} 
% &$Anc(k)$ 	& Ancestors of node $k$ in $E$								\\
% \midrule
% &$n$		& \specialcell{Dimension of the  matrix $A$}						\\
% % &$nlevel$	& Height of  $E$ $\bigo{\log n}$ 								\\
% &$l$		&  $\log_{2} P_{z}$									\\
% % &$M$		& \specialcell{Per-process memory }					\\
% &$W$		& Communication cost								\\
% &$V$		& Per-process communication volume								\\
% &$\alpha$   & Cost of initiating a data transfer		\\
% &$\beta$    & Cost of transferring a unit data		\\
% \multirow{-7}{*}{Misc.}
% &$\gamma$   & Number of right hand sides		\\

% \bottomrule

% \end{tabular}
% \end{table}

